TAMBRIDGE: Bridging Frame-Centered Tracking and 3D Gaussian Splatting for Enhanced SLAM

The limited robustness of 3D Gaussian Splatting (3DGS) to motion blur and camera noise, along with its poor real-time performance, restricts its application in robotic SLAM tasks. Upon analysis, the primary causes of these issues are the density of views with motion blur and the cumulative errors in dense pose estimation from calculating losses based on noisy original images and rendering results, which increase the difficulty of 3DGS rendering convergence. Thus, a cutting-edge 3DGS-based SLAM system is introduced, leveraging the efficiency and flexibility of 3DGS to achieve real-time performance while remaining robust against sensor noise, motion blur, and the challenges posed by long-session SLAM. Central to this approach is the Fusion Bridge module, which seamlessly integrates tracking-centered ORB Visual Odometry with mapping-centered online 3DGS. Precise pose initialization is enabled by this module through joint optimization of re-projection and rendering loss, as well as strategic view selection, enhancing rendering convergence in large-scale scenes. Extensive experiments demonstrate state-of-the-art rendering quality and localization accuracy, positioning this system as a promising solution for real-world robotics applications that require stable, near-real-time performance. Our project is available at https://ZeldaFromHeaven.github.io/TAMBRIDGE/

==> 01_introduction_pre.tex <==

\section{Introduction}
The capability of achieving real-time location and high-fidelity mapping simultaneously (SLAM) without any prior knowledge of an unknown scene is significant to intelligent robots in establishing a high-level understanding of the environment just in time. During the past two decades, the computational consumption balance between tracking accuracy and mapping fidelity has always been a significant topic because the more dense a map is, the more noisy it will be for tracking and will be more time-consuming.

Plenty of trials on picking up a proper, consistent representation of the scene have been taken to find an appropriate representation that can give high-level scene understanding, be beneficial for tracking and be less time-consuming. Such work can be categorized into tracking-centered representation and mapping-centered representation. The work of building a tracking-centered representation takes over in earlier times. They mainly focus on the scene representation beneficial for more accurate tracking like feature point clouds~\cite{klein2007parallel,davison2007monoslam, Mur-Artal2017ORB-SLAM2:Cameras}, surfels~\cite{whelan2015elasticfusion,schops2019bad}, depth maps~\cite{stuhmer2010real,newcombe2011dtam}, or implicit representations~\cite{newcombe2011kinectfusion,niessner2013voxel_hashing,dai2017bundlefusion} in a relatively sparse way. Thanks to the rapid development of computation resources, building a global consistent, high-fidelity and tracking-beneficial representation is affordable based on the new formulation in recent works. The typical technology is  neural radiance fields that allow for high-fidelity view-synthesis using the implicit representation based on neural network indication. A growing body of dense neural SLAM methods~\cite{Sucar2021IMAP:Real-Time,huang2021di,zhu2022nice,mahdi2022eslam,tang2023mips,wang2023co,sandstrom2023point,zhang2023go} has been developed to build a high-fidelity map with the same tracking accuracy as tracking-centered works.

Despite the advancements made by NeRF-based SLAM methods in finding a suitable scene representation that enhances tracking accuracy and facilitates high-fidelity scene rendering, they still encounter challenges related to time-consuming optimization convergence. Additionally, they are only applicable in small synthetic scenes with minimal sensor noise and motion blur. Consequently, achieving robustness and real-time performance remains an unresolved issue for mapping-centered SLAM.

To solve the time consuming problem, the advent of 3DGS  based SLAM can render the scene in  faster speed and higher quality than NeRF, using Gaussian Splatting algorithm which is differetiable and more easy to convergence without neural network. What's more, such methods are interpretible as well as manipulatable. However, to the best of our knowledge,  recent 3DGS based SLAM system still has real-time performance problem since no work could achieve a steady performance over 5FPS in real scene. What's more, the application of 3GDS based SLAM is still limited into small scenes and is quite  unrobust towards sensor noise and motion blur, which means that they are not competent in long term robot mission.

Our work aims to take a further step into solving the time-consuming and robustness problem of mapping-centered SLAM by combining the advantages of tracking-centered noiseless pose estimation and mapping-centered high-fidelity scene representation. Based on this idea, we adapt an ORB based VO as our front-end to achieve real-time and high-accuracy tracking. Then, we use a fusion bridge to filter the view point sending to the  back-end as well as using a union optimezation method based on reprojection error and rendering error to get a better pose initialization for online 3DGS based mappping. In the backend, we adapt a 3DGS based online rendering algorithm to  map and render the 3DGS based on the fine selected and initialized pose obtained from the fusion  bridge. The experiment results on real indoor scenes taken by robot system shows that our system could achieve a steady 5+FPS real-time performance as well as good rendering quality and new-view synthesized capability even in long term robot mission, which to our knowledge is the first 3DGS based SLAM system could achieve steady real-time perforance on robot mission regardless of noise and distance.

In summary, our contribution are as follow:
\begin{enumerate}
    \item Discover the importance of good rendering pose initialization and the choice of view selection to make online 3dgs easy to convergent especially in large-scale scene.
    \item Implement a plug and play fusion bridge module that could fuse feature based SLAM front-ends with online 3dgs based back-ends
    \item The first 3dgs based SLAM System that could achieve real-time tracking, mapping and rendering and competent to long distance robot SLAM mission.
\end{enumerate}








==> 02_related_work.tex <==
\section{Related Works}
Visual SLAM can be categorized into two paradigms based on the significance of localization and mapping within the system: the frame-centered SLAM paradigm and the map-centered SLAM paradigm.

\subsection{Frame-centered SLAM  paradigm}

The frame-centered SLAM paradigm operates by extracting features from images that possess rotational invariance, translational invariance, scale invariance, or photometric invariance—such as points, planes, or blocks. It minimizes reprojection errors or photometric errors across consecutive frames through various levels of data association, jointly optimizing environment depth information and pose transformations.

The lightweight and sparse nature of feature extraction allows for rapid and efficient pose tracking, with minimal time and spatial overhead. Long-standing design for feature robustness and optimized data association across different stages enable the frame-centered SLAM paradigm to estimate poses with greater accuracy and robustness. The multi-threaded design ensures the parallelism of local and global geometries. Thus, sparse tracking features, robust optimization algorithms, and a parallel global framework make the frame-centered SLAM paradigm widely applicable in long-term SLAM tasks for mobile robots.

ORB-SLAM, a well-known implementation within the frame-centered SLAM systems, utilizes sparse ORB manual features and a multi-stage data association algorithm to refine poses from coarse to fine. Its tri-threaded architecture for tracking, local mapping, and loop closure, with a keyframe sequence as the medium of information between threads, enables the system to achieve robust, real-time, and precise visual localization. It is extensively used in applications like robotics, where robustness is crucial.

However, due to the sparsity of the features, frame-centered SLAM paradigms typically generate maps primarily for localization purposes and lack a comprehensive understanding and modeling of the scene. Therefore, they are unable to provide sufficient environmental information for downstream tasks, limiting their ability to support higher-level scene understanding and modeling.

\subsection{Map-centered SLAM paradigm}
The map-centered SLAM paradigm emphasizes the unity of 3D representation within the framework and leverages global information through consistently reconstructed 3D maps from tracking data.

To capture scenes with photorealistic fidelity, differentiable volumetric rendering has recently become popular, driven by the widespread adoption of neural radiance fields (NeRF)\cite{mildenhall2021nerf}. Techniques using this approach perform volumetric rendering by progressing along pixel rays and querying a single multilayer perceptron (MLP) for opacity and color, optimizing the MLP to minimize rendering losses using multiview information for high-quality 3D reconstruction and precise tracking. However, these methods require considerable training time due to their complexity.

Given the high training costs of neural networks and the difficulty in editing implicit neural representations, explicit volumetric representations such as multi-resolution voxel grids\cite{fridovich2022plenoxels,Zhu2022CVPR,liu2020neural} or hashing functions \cite{mueller2022instant}have become research focal points to enhance performance. For instance, Point-NeRF \cite{xu2022point}implements volumetric rendering through neural point clouds and feature interpolation, offering faster and more effective 3D reconstruction suitable for robotics applications, although its efficiency still revolves around ray and volumetric ray sampling. Analysis of these projects has shown that the main contributor to high-quality novel view synthesis is not the neural network, but the differentiable volumetric rendering, and it is possible to achieve comparable rendering quality to NeRF without using MLPs.

Leveraging 3D Gaussian Splatting (3DGS) as the sole underlying scene representation adopts the efficiency, locality, and ease of deformation or modification of the aforementioned explicit volumetric representations, representing geometry in a smooth, continuously differentiable manner. By implementing differentiable rasterization in place of NeRF’s per-pixel ray marching, fast and high-fidelity rendering of scenes is achieved.

Initiatives like SplaTAM, MonoGS, and GS-SLAM have pioneered these methods. SplaTAM, as the first open-source solution, uses isotropic 3D Gaussian ellipsoids as the scene representation, achieving scene reconstruction through rapid differentiable rasterization via 3DGS. It divides the SLAM process into localization, densification, and mapping phases, achieving localization accuracy comparable to NeRF-based methods and far superior scene reconstruction capabilities. However, the localization phase, which uses per-pixel color-depth rendering photometric errors for gradient descent-based pose optimization, exhibits significant sensitivity to motion blur, substantial depth noise, and aggressive rotations in real indoor scenes, as well as large time overheads in localization and mapping, preventing real-time applications in robot proprioceptive and scene perception tasks.

Similarly, MonoGS adopts a comparable framework, deriving analytic Jacobian determinants, Gaussian shape regularization, and geometric verification formulas for camera pose estimation, expanding 3DGS-based SLAM input from RGBD to monocular with competitive capabilities. Like SplaTAM, it significantly exceeds the reconstruction performance of NeRF-based SLAM but remains sensitive to motion blur, substantial depth noise, and violent rotations, with its per-pixel photometric and geometric residuals substantially increasing the time overhead for localization and exhibiting poor robustness to noise.

\subsection{Fusion SLAM paradigm}
Orbeez \cite{chung2023orbeezslam} exemplifies a classical case of the integration of frame-centered and map-centered SLAM paradigms. This system employs a feature-based SLAM front-end (ORB-SLAM) to obtain precise poses, while concurrently updating a NeRF neural network backend based on the Instant-NGP framework for map rendering. This setup validates that the visual odometry from ORB-SLAM2 can provide superior camera pose estimates for the backend NeRF training, which operates without the need for pre-training and can run in real-time online. Consequently, Orbeez-SLAM serves as a successful example of paradigm fusion, rendering dense environmental and color information while maintaining precise pose acquisition. It is capable of handling various indoor scenarios with performance in speed, localization, and reconstruction that surpasses that of NeRF-SLAM, which solely relies on a map-centered paradigm.

==> checklist.tex <==
\newpage
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justification{The contributions are mentioned in \ref{intro}, which matches the theoretical and experimental results in \ref{method} and \ref{experiment}, respectively. The results can be expected to generalize to other settings, besides the test on TUM RGB-D, we also adapt our test in our laboratory meeting room, and you can find the qualitative and quantitative results in \ref{lab}.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justification{We have our "Limitation" section in \ref{limi}, where we will give a further explanation about the limitations of our method~\ref{limi-method} and experiment~\ref{limi-experiment}. In~\ref{experiment}, we have already declared the robustness of our method towards motion blur and sensor noise. We conducted our experiments using only one dataset, which might be seen as a limitation. To address this, we clarified our rationale in the checklists: the TUM RGB-D dataset includes up to 18 sequences collected by robots and handheld devices, featuring significant motion blur and sensor noise. This dataset effectively simulates typical indoor scenarios, aligning well with our objectives. Additionally, we did not use any synthetic datasets like Replica, which are commonly used in other NeRF-based SLAM and 3DGS-SLAM studies, because these datasets lack motion blur and random sensor noise, failing to replicate real-world robotic conditions. Instead, we supported our method's effectiveness with results from other sequences within the TUM RGB-D dataset. The computational efficiency is one of our key contributions, and it's declared in \ref{ablations} as well as in \ref{FPS} where the hyper-parameter values associated with the curves are labeled.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justification{All the theorems and formulas in the paper are numbered and cross-referenced in \ref{method}. All the formulas are stated in a clear and detailed way.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justification{The code is currently being optimized and will be open-sourced on GitHub when ready. Although it is not yet publicly available, the reproducibility of our experimental data is assured. We have provided all hyperparameter values in the supplementary materials~\ref{app:ei} and have comprehensively detailed our overall framework, the specifics of each module, and all involved formulas in the methods section~\ref{method}.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justification{Due to the substantial amount of code, we are currently optimizing it. We fully understand the value of open-source code in the SLAM field, so once the optimization is complete, we will release it on our GitHub project page. To facilitate system reproduction, we have provided complete hyperparameter values and have detailed the implementation in the methods~\ref{method} section through formulas, descriptions, and figures.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justification{In the experimental section~\ref{experiment}, we have detailed the implementation specifics, including hardware, programming language, use of open-source modules, and optimizer settings. Additionally, in the appendix\ref{app:ei}, we have disclosed the hyperparameter values and provided curves showing their impact on frame rate and reconstruction quality.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justification{In the SLAM field, it is uncommon to provide error bars because the results typically exhibit considerable stability upon reproduction, especially for SLAM systems like ours that do not incorporate neural networks. However, to give readers a clearer understanding of the variations in reconstruction quality, we have included error bars in the figures~\ref{17}~\ref{18}~\ref{19} in the Appendix section~\ref{app:ei}. These error bars represent the standard deviation of the reconstruction results, and we have annotated them in the figures accordingly.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justification{In the experimental section, we clearly state that all experiments~\ref{experiment} were conducted on a single NVIDIA RTX 3090 GPU. The total frame rate of the system for each sequence is provided in the experimental tables. Given that near-real-time performance is one of our core contributions, we have included detailed frame rate-quality curves~\ref{fig:FPS}. Additionally, we provide frame rate information in the demo video included in the supplementary materials.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justification{All our submitted materials ensure anonymity and comply with the NeurIPS Code of Ethics.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justification{Our work has no societal impact. Our model cannot generate false information; all components are interpretable and based on rigorous mathematical derivations. Additionally, it does not involve security or privacy issues. However, it is important to note that in robot applications, the new view points generated by 3DGS may not fully align with actual perspectives, potentially causing misalignment or displacement. Therefore, caution is advised when using it in scenarios that may lead to safety incidents.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justification{The paper poses no such risks.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justification{In references, we have cited the the original paper that produced the code package~\cite{ORBSLAM3_TRO}~\cite{keetha2023splatam} or dataset~\cite{dataset2012tum}. The package~\cite{ORBSLAM3_TRO} uses a GPL-3.0  License (\url{https://github.com/UZ-SLAMLab/ORB_SLAM3?tab=GPL-3.0-1-ov-file#readme}), the ~\cite{keetha2023splatam} uses a BSD-3-Clause License (\url{https://github.com/spla-tam/SplaTAM?tab=BSD-3-Clause-1-ov-file#readme}} and the dataset ~\cite{dataset2012tum} uses a CC BY 4.0 License (\url{https://paperswithcode.com/dataset/tum-rgb-d}).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justification{The paper does not release new assets.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justification{The paper does not involve crowdsourcing nor research with human subjects.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justification{The paper does not involve crowdsourcing nor research with
human subjects.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}



==> rendering_old.tex <==
\begin{table}[htbp]
\centering
\scriptsize
\caption{\textbf{Tracking and Rendering Performance on TUM-RGBD~\cite{sturm2012benchmark}.} }
%We outperform existing dense neural RGBD methods and SplaTAM on the commonly reported tracking and rendering metrics. Also, We outperform SplaTAM on the commonly reported tracking metrics and are on par with the current state-of-the-art SplaTAM on rendering metrics.
\setlength\tabcolsep{2.3mm}
\begin{tabular}{lcccccc}
\toprule
Method & Metric & \texttt{fr1/desk} & \texttt{fr2/xyz} & \texttt{fr3/office} & Avg.\\
\midrule
\multirow{5}{*}{\makecell[l]{ORB-SLAM3~\cite{ORBSLAM3_TRO}}}
& RMSE$\downarrow$ & 2.06 & 0.33 & 1.04 & 1.14 \\
& PSNR$\uparrow$ & -- & -- & -- & -- \\
& SSIM$\uparrow$ & -- & -- & -- & -- \\
& LPIPS$\downarrow$ & -- & -- & -- &--\\  \hline
\multirow{5}{*}{\makecell[l]{NICE-SLAM~\cite{Zhu2022CVPR}}}
& RMSE$\downarrow$ & 4.26 & 34.49 & 3.87 & 14.21 \\
& PSNR$\uparrow$ & 13.83 & \rd17.87 & 12.890 & 14.86 \\
& SSIM$\uparrow$ & 0.569 & 0.718 & 0.554 & 0.614 \\
& LPIPS$\downarrow$ & 0.482 & \rd0.344 & 0.498 & \rd0.441 \\[0.8pt] \hdashline \noalign{\vskip 1pt}
\multirow{5}{*}{\makecell[l]{Vox-Fusion~\cite{yang2022vox}}}
& RMSE$\downarrow$ &3.52 &  1.49 & 26.01 & 10.34\\
& PSNR$\uparrow$ & 15.79 & 16.32 & 17.27 & 16.46 \\
& SSIM$\uparrow$ & 0.647 & 0.706 & 0.677 & 0.677 \\
& LPIPS$\downarrow$ & 0.523 & 0.433 & 0.456 & 0.471 \\ [0.8pt] \hdashline \noalign{\vskip 1pt}
\multirow{5}{*}{\makecell[l]{Point-SLAM~\cite{xu2022point}}}
& RMSE$\downarrow$ &4.34 &  31.73 & 3.87 & 13.31\\
& PSNR$\uparrow$ & \rd13.87 & 17.56 & \rd18.43 & \rd16.62 \\
& SSIM$\uparrow$ & 0.627 & \rd0.708 & \rd0.754 & \rd0.696 \\
& LPIPS$\downarrow$ & 0.544 & 0.585 & \rd0.448 & 0.526 \\[0.8pt] \hline \noalign{\vskip 1pt}
\multirow{5}{*}{\makecell[l]{SplaTAM\textcolor{red}{$^*$}~\cite{keetha2024splatam}}}
& RMSE$\downarrow$ &3.38 &  1.34 & 5.03 & 3.25\\
& PSNR$\uparrow$ & \nd\textbf{22.00} & \nd\textbf{24.50} & \nd\textbf{21.90} & \nd\textbf{22.80} \\
& SSIM$\uparrow$ & \nd0.857 & \fs\textbf{0.947} & \nd\textbf{0.876} & \nd\textbf{0.893} \\
& LPIPS$\downarrow$ & \nd0.232 & \fs\textbf{0.100} & \nd\textbf{0.202} & \nd\textbf{0.178} \\ [0.8pt] \hdashline \noalign{\vskip 1pt}
\multirow{5}{*}{\makecell[l]{TAMBridge (ours)}}
& RMSE$\downarrow$ &\textbf{1.75} &  \textbf{0.32} & \textbf{1.42} & \textbf{1.16}\\
& PSNR$\uparrow$ & 21.22 & 23.44 & 20.15 & 21.60 \\
& SSIM$\uparrow$ & \textbf{0.88} & 0.90 & 0.82 & 0.87 \\
& LPIPS$\downarrow$ &\textbf{0.19 }& \nd\textbf{0.100} & 0.25 & 0.18 \\[0.8pt]  \noalign{\vskip 1pt}
\bottomrule
\end{tabular}
\label{tab:tum_rendering}
\end{table}

\begin{table}[!htb]
\centering
\scriptsize
\caption{\textbf{Tracking and Rendering Performance on TUM-RGBD~\cite{sturm2012benchmark} mobile slam sequence}. Convergence failure is represented by "\xmark" .}
\begin{tabularx}{\textwidth}{lXXXXXX}
\toprule
Method & Metric & \texttt{fr2/360} & \texttt{fr2/slam} & \texttt{fr2/slam2} & Avg.\\
\midrule
\multirow{4}{*}{\makecell[l]{ORB-SLAM3~\cite{ORBSLAM3_TRO}}}
& RMSE$\downarrow$ & 108.67 & 167.63 & 150.98 & 142.43 \\
& PSNR$\uparrow$ & -- & -- & --  & --\\
& SSIM$\uparrow$ & -- & -- & --  & --\\
& LPIPS$\downarrow$ & -- & -- & -- & --\\  \hdashline
\multirow{4}{*}{\makecell[l]{SplaTAM\textcolor{red}{$^*$}~\cite{keetha2024splatam}}}
& RMSE$\downarrow$ &101.37 &  \xmark & 627.31 & \xmark\\
& PSNR$\uparrow$ & \textbf{24.33} & \xmark &13.62 & \xmark \\
& SSIM$\uparrow$ &\textbf{0.82 } &\xmark &0.42 & \xmark \\
& LPIPS$\downarrow$ &\textbf{0.22} & \xmark & 0.54&\xmark \\ [0.8pt] \hdashline \noalign{\vskip 1pt}
\multirow{4}{*}{\makecell[l]{TAMBridge (ours)}}
& RMSE$\downarrow$ &\textbf{8.43} &  \textbf{10.06} &\textbf{ 6.7} &\textbf{8.40}\\
& PSNR$\uparrow$ & 24.32 & \textbf{23.54} &\textbf{24.52} & \textbf{24.14} \\
& SSIM$\uparrow$ &0.79 & \textbf{0.8} & \textbf{0.82} & \textbf{0.80} \\
& LPIPS$\downarrow$&0.24&\textbf{0.24} & \textbf{0.19}& \textbf{0.22} \\[0.8pt]  \noalign{\vskip 1pt}
\bottomrule
\end{tabularx}
\label{tab:tum_mobile}
\end{table}
